From Obstacles to Resources: Semi-supervised Learning Faces Synthetic Data Contamination

Semi-supervised learning (SSL) can improve model performance by leveraging unlabeled images, which can be collected from public image sources with low costs. In recent years, synthetic images have become increasingly common in public image sources due to rapid advances in generative models. Therefore, it is becoming inevitable to include existing synthetic images in the unlabeled data for SSL. How this kind of contamination will affect SSL remains unexplored. In this paper, we introduce a new task, Real-Synthetic Hybrid SSL (RS-SSL), to investigate the impact of unlabeled data contaminated by synthetic images for SSL. First, we set up a new RS-SSL benchmark to evaluate current SSL methods and found they struggled to improve by unlabeled synthetic images, sometimes even negatively affected. To this end, we propose RSMatch, a novel SSL method specifically designed to handle the challenges of RS-SSL. RSMatch effectively identifies unlabeled synthetic data and further utilizes them for improvement. Extensive experimental results show that RSMatch can transfer synthetic unlabeled data from `obstacles' to `resources.' The effectiveness is further verified through ablation studies and visualization.

==> tabs/table_sup1.tex <==
\begin{table*}[t]
\centering
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c}
\toprule
& Hyper-parameter & Description  & CIFAR-10 & CIFAR100 & TinyImageNet & ImageNet \\
\midrule
\multirow{9}{*}{\rotatebox{90}{SSL~(FixMatch)}} & $\tau$ & SSL confidence threshold & \multicolumn{4}{c}{0.95} \\
 & $\lambda$ & Unsupervised loss weight & \multicolumn{4}{c}{1} \\
 & $\beta$ & Momentum & \multicolumn{4}{c}{0.9} \\
 & $\alpha$ & EMA weight & \multicolumn{4}{c}{0.999} \\
 & $lr$ & Learning rate & \multicolumn{4}{c}{0.03} \\
 & $B$ & Labeled data batch size & \multicolumn{4}{c}{64} \\
 & Iteration & Training iterations & \multicolumn{4}{c}{$2^{20}$} \\
 \cmidrule{2-7}
& $\mu$ & Unlabeled data batch ratio & 7 & 7 & 7 & 1 \\
 & Weight decay & Weight decay & 0.0005 & 0.001 & 0.0005 & 0.0001\\
\midrule
\multirow{3}{*}{\rotatebox{90}{Ours}} & $N_q$ & The sub-queue size of CSQueue  & \multicolumn{4}{c}{8} \\
 & $P$ & The selected sub-queue number for each iteration  & \multicolumn{4}{c}{10} \\
 & $Q$ & The enqueued number for each iteration  & \multicolumn{4}{c}{1} \\
 \bottomrule
\end{tabular}
}
\end{center}
\caption{Hyper-parameters of RSMatch with FixMatch as the basic SSL method.}
\label{tab:tab_sup_1}
\end{table*}

==> tabs/table_sup2.tex <==
\begin{table}[t]
\centering
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccc}
\toprule
Dataset & \multicolumn{3}{c}{CIFAR-10} \\
\midrule
Synthetic ratio ($\alpha$) & 0.3 & 0.5 & 1.0 \\
\midrule
Ours-FixMatch &  92.45\scalebox{0.8}{$\pm$1.7} & 97.28\scalebox{0.8}{$\pm$2.6} & 97.53\scalebox{0.8}{$\pm$0.8} \\
Ours-FlexMatch &  92.05\scalebox{0.8}{$\pm$0.8} & 92.82\scalebox{0.8}{$\pm$0.4} & 85.93\scalebox{0.8}{$\pm$2.1} \\
Ours-SoftMatch &  94.30\scalebox{0.8}{$\pm$1.1} & 96.42\scalebox{0.8}{$\pm$0.3} & 87.51\scalebox{0.8}{$\pm$0.7} \\
\bottomrule
\end{tabular}
}

\vspace{10pt}

\resizebox{\linewidth}{!}{
\vspace{20pt}
\begin{tabular}{l|ccc}
\toprule
Dataset & \multicolumn{3}{c}{CIFAR-100} \\
\midrule
Synthetic ratio ($\alpha$) & 0.3 & 0.5 & 1.0 \\
\midrule
Ours-FixMatch &  90.27\scalebox{0.8}{$\pm$1.5} & 93.79\scalebox{0.8}{$\pm$0.2} & 96.74\scalebox{0.8}{$\pm$1.5} \\
Ours-FlexMatch &  90.93\scalebox{0.8}{$\pm$1.4} & 94.15\scalebox{0.8}{$\pm$0.6} & 94.28\scalebox{0.8}{$\pm$0.3} \\
Ours-SoftMatch &  85.93\scalebox{0.8}{$\pm$3.3} & 88.94\scalebox{0.8}{$\pm$0.8} & 95.97\scalebox{0.8}{$\pm$1.6} \\
\bottomrule
\end{tabular}
}

\vspace{10pt}

\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccc|c}
\toprule
Dataset & \multicolumn{3}{c|}{TinyImageNet} & ImageNet\\
\midrule
Synthetic ratio ($\alpha$) & 0.3 & 0.5 & 1.0 & 0.5 \\
\midrule
Ours-FixMatch &  94.44\scalebox{0.8}{$\pm$2.7} & 94.79\scalebox{0.8}{$\pm$1.4} & 97.97\scalebox{0.8}{$\pm$1.2} & 96.87\scalebox{0.8}{$\pm$2.0} \\
\bottomrule
\end{tabular}
}
\end{center}
\caption{Deepfake detection accuracy (\%) with various synthetic ratios $\alpha$ on CIFAR-10~\cite{krizhevsky2009learning}, CIFAR-100~\cite{krizhevsky2009learning} with 25 labels per class and TinyImageNet~\cite{deng2009imagenet}, ImageNet~\cite{deng2009imagenet} with 10\% labels per class.}
\label{tab:tab_sup_2}
\end{table}
